Learning Models of Individual Behavior in Chess

AI systems that can capture human-like behavior are becoming increasingly useful in situations where humans may want to learn from these systems, collaborate with them, or engage with them as partners for an extended duration. In order to develop human-oriented AI systems, the problem of predicting human actions -- as opposed to predicting optimal actions -- has received considerable attention. Existing work has focused on capturing human behavior in an aggregate sense, which potentially limits the benefit any particular individual could gain from interaction with these systems. We extend this line of work by developing highly accurate predictive models of individual human behavior in chess. Chess is a rich domain for exploring human-AI interaction because it combines a unique set of properties: AI systems achieved superhuman performance many years ago, and yet humans still interact with them closely, both as opponents and as preparation tools, and there is an enormous corpus of recorded data on individual player games. Starting with Maia, an open-source version of AlphaZero trained on a population of human players, we demonstrate that we can significantly improve prediction accuracy of a particular player's moves by applying a series of fine-tuning methods. Furthermore, our personalized models can be used to perform stylometry -- predicting who made a given set of moves -- indicating that they capture human decision-making at an individual level. Our work demonstrates a way to bring AI systems into better alignment with the behavior of individual people, which could lead to large improvements in human-AI interaction.

==> chess_examples/out.tex <==
\newgame
\resetPgnTags
\def\Event{}
\def\Site{}
\def\Date{}
\def\WhitePlayer{Human}
\def\BlackPlayer{Transfer Maia}
\def\Result{\whiteWins}
\def\Eco{C13}
\gameHeader

\gameskip
\mainline{%
 1. e4 1... e6 2. d4 2... d5 3. Nc3 3... Nf6 4. Bg5 4... Be7 5. e5 5... Nfd7 6. h4 6... c5?! } [\movecomment{%
6... Bxg5 7. hxg5 Qxg5 8. Nh3 Qh4 9. g3 Qe7 10. Qg4 g6 11. O-O-O}]
\mainline{%
7. Nb5?? } [\movecomment{%
7. Bxe7 Kxe7 8. f4 Nc6 9. dxc5 Nxc5 10. a3 a5 11. Qg4 Nd4}]
\mainline{%
7... O-O?? } [\movecomment{%
7... f6 8. exf6 Nxf6 9. dxc5 O-O 10. Nf3 Bxc5 11. Qd2 Qb6 12. b4}]
\mainline{%
8. Bxe7 8... Qxe7 9. Nc7 9... Nc6 10. Nxa8 10... Nxd4 11. c3 11... Nc6 12. f4 12... f6 13. exf6? } [\movecomment{%
13. Nf3 fxe5}]
\mainline{%
13... Nxf6 14. Nf3 14... Nh5?? } [\movecomment{%
14... e5 15. Be2}]
\mainline{%
15. Qd2 15... Nxf4 16. O-O-O 16... Bd7?! } [\movecomment{%
16... c4 17. Re1}]
\mainline{%
17. Nc7 17... Qd6 18. Nb5 18... Qb8 19. Bd3 19... a6 20. Na3 20... b5 21. Ng5 21... h6 22. Nf3?! } [\movecomment{%
22. Bh7+}]
\mainline{%
22... b4 23. cxb4?! } [\movecomment{%
23. Nc2 c4}]
\mainline{%
23... Nxb4 24. Bb1 24... e5 25. Rhe1?? } [\movecomment{%
25. g3}]
\mainline{%
25... e4 26. Ng1? } [\movecomment{%
26. Qc3}]
\mainline{%
26... Qe5?? } [\movecomment{%
26... Bg4 27. Nh3 Nbd3+ 28. Bxd3 Nxd3+ 29. Kb1 Bxd1 30. Rxd1 c4 31. Qc2 Kh8 32. Ka1 Qe5 33. Nb1}]
\mainline{%
27. Qc3?? } [\movecomment{%
27. g3 Ne6 28. Nc4 Qc7 29. Rxe4 dxe4 30. Qxd7 Nd3+ 31. Rxd3 Rf1+ 32. Kd2 exd3 33. Qxe6+ Qf7}]
\mainline{%
27... Qxc3+?? } [\movecomment{%
27... Qb8 28. Nc4}]
\mainline{%
28. bxc3 28... Nbd3+ 29. Bxd3 29... Nxd3+ 30. Kd2 30... Rf2+?! } [\movecomment{%
30... Bg4 31. Ke3}]
\mainline{%
31. Re2 31... Bg4?? } [\movecomment{%
31... Rf4 32. Nh3}]
\mainline{%
32. Rxf2 32... Nxf2 33. Rb1 33... d4 34. Rb8+ 34... Kh7 35. cxd4 35... cxd4 36. Nc4 36... e3+?! } [\movecomment{%
36... Be6 37. Ne5 Bxa2 38. Rd8 e3+ 39. Ke2 Ne4 40. Rxd4 Ng3+ 41. Ke1 Nf5 42. Rf4 Nd6 43. Ra4}]
\mainline{%
37. Nxe3 37... dxe3+ 38. Kxe3 38... Nd1+ 39. Kd2 39... Nf2 40. Re8 40... Kg6 41. Nf3 41... Kf7 42. Re2 42... Nh1 43. Ne5+ 43... Kf6 44. Nxg4+ 44... Kf5 45. Ne3+ 45... Kf4 46. Nd5+ 46... Kg3 47. Re7 47... Kxh4?? } [\movecomment{%
47... Kxg2 48. Rxg7+}]
\mainline{%
48. Rxg7 48... Ng3 49. Rg6 49... h5?! } [\movecomment{%
49... Nf5 50. Ne3}]
\mainline{%
50. Rxa6? } [\movecomment{%
50. Ne3 Ne4+ 51. Kd3 Ng5 52. a4 Kg3 53. Rxg5+ Kf4 54. Rf5+ Kg3 55. Rf6 a5 56. Rf5 Kh4}]
\mainline{%
50... Kg4 51. Ne3+ 51... Kf4 52. Ra4+ 52... Ke5 53. Ra5+ 53... Kf4 54. a4 54... Ne4+ 55. Ke2 55... Nc3+ 56. Kd3 56... Ne4?! } [\movecomment{%
56... Na2 57. Rf5+}]
\mainline{%
57. Rxh5?! } [\movecomment{%
57. Rf5+ Kg3 58. Kxe4 Kh4 59. a5 Kg3 60. a6 Kh4 61. a7 Kg3 62. a8Q Kh4 63. Qa1 Kg3}]
\mainline{%
57... Ng3?! } [\movecomment{%
57... Nd6 58. a5 Kg3 59. Nf5+ Kg4 60. Nxd6 Kxh5 61. a6 Kg5 62. a7 Kf6 63. a8Q Ke6 64. Ne4}]
\mainline{%
58. Rh4+ 58... Ke5 59. a5 59... Nf5 60. Rh5 60... Ke6 61. Rxf5 61... Kd6 62. a6 62... Kc7 63. a7 63... Kb7 64. Rf7+ 64... Ka8 65. Rf6 65... Kxa7 66. Kc4 66... Kb7 67. Kd5 67... Kc7 68. g4 68... Kd7 69. g5 69... Ke7 70. Ke5 70... Kd7 71. Nd5 71... Ke8 72. Kd6 72... Kd8 73. Rf8\mate{}}\rwwins

\gameskip
\newgame
\resetPgnTags
\def\Event{}
\def\Site{}
\def\Date{}
\def\WhitePlayer{Transfer Maia}
\def\BlackPlayer{Human}
\def\Eco{B00}
\gameHeader

\gameskip
\mainline{%
 1. e4 1... a6 2. d4 2... b5 3. Nf3 3... Bb7 4. Nc3? } [\movecomment{%
4. Bd3 e6 5. O-O c5 6. c3 cxd4 7. cxd4 Nf6 8. Nbd2 Be7}]
\mainline{%
4... b4 5. Nd5 5... e6 6. Nf4 6... Bxe4 7. Bd3 7... Nf6 8. O-O 8... Be7 9. Re1 9... Bxd3 10. Qxd3 10... O-O 11. Bd2 11... Nc6?! } [\movecomment{%
11... a5 12. a3 bxa3 13. bxa3 h6 14. Rab1 d6 15. Qb5 Qd7 16. c4 Qxb5 17. Rxb5 a4 18. Reb1}]
\mainline{%
12. Rad1?! } [\movecomment{%
12. d5}]
\mainline{%
12... a5? } [\movecomment{%
12... Bd6 13. c4 bxc3 14. bxc3 Rb8 15. Bc1 a5 16. c4 Bb4 17. Rf1 d5 18. Ne5 dxc4 19. Qxc4}]
\mainline{%
13. c4? } [\movecomment{%
13. d5 Nb8}]
\mainline{%
13... bxc3 14. Bxc3? } [\movecomment{%
14. bxc3 d5 15. Ng5 Bd6 16. Nh5 g6 17. Nf4 Re8 18. Qh3 Rb8 19. Nd3 e5 20. Nxe5 Nxe5}]
\mainline{%
14... Re8?! } [\movecomment{%
14... Nb4}]
\mainline{%
15. d5 15... exd5?? } [\movecomment{%
15... Nb4 16. Bxb4 axb4 17. dxe6 fxe6 18. Qc4 Bd6 19. Nd3 Nd5 20. Nde5 c6 21. Re2 Rf8 22. g3}]
\mainline{%
16. Nxd5 16... Nxd5 17. Qxd5 17... Bd6?? } [\movecomment{%
17... h6 18. Ne5 Nxe5 19. Qxe5 Bf6 20. Qxe8+ Qxe8 21. Rxe8+ Rxe8 22. Bxa5 Bxb2 23. Rxd7 Ra8 24. Bxc7}]
\mainline{%
18. Rxe8+?? } [\movecomment{%
18. Ng5 Rf8}]
\mainline{%
18... Qxe8 19. Re1 19... Qf8?! } [\movecomment{%
19... Ne7}]
\mainline{%
20. Ng5? } [\movecomment{%
20. Qf5 Ne7 21. Qxd7 a4 22. a3 Nd5 23. Ba5 Nb6 24. Qc6 Bc5 25. Bxb6 cxb6 26. Re4 Qd8}]
\mainline{%
20... h6 21. Ne4 21... Re8 22. g3?! } [\movecomment{%
22. Kf1 Re6 23. a3 Qb8 24. Nxd6 Rxd6 25. Qc4 Re6 26. Rxe6 fxe6 27. Qd3 Qe8 28. Qa6 Qb8}]
\mainline{%
22... Nb4?? } [\movecomment{%
22... Re7 23. Kf1}]
\mainline{%
23. Qd4?! } [\movecomment{%
23. Qxa5}]
\mainline{%
23... Be5 24. Qxd7 24... Bxc3?? } [\movecomment{%
24... Re7 25. Qd2 Bxc3 26. Nxc3 Rxe1+ 27. Qxe1 Qd8 28. Qe4 c6 29. a3 Nd3 30. Qxc6 Nxb2 31. Qe4}]
\mainline{%
25. bxc3?? } [\movecomment{%
25. Nf6+}]
\mainline{%
25... Rd8 26. Qxc7 26... Nd3 27. Rb1?? } [\movecomment{%
27. Rd1}]
\mainline{%
27... Rc8?? } [\movecomment{%
27... f5 28. Nd2 Nxf2 29. Nf3 Nh3+ 30. Kg2 Ng5 31. Nd4 Rc8 32. Qd7 Rxc3 33. Rb7 Qf6 34. Qxf5}]
\mainline{%
28. Qxa5 28... Ra8? } [\movecomment{%
28... Qe7 29. Qf5}]
\mainline{%
29. Qd5?! } [\movecomment{%
29. Qb5 Rd8 30. Rd1 Qe8 31. Qxe8+ Rxe8 32. Nd6 Nb2 33. Nxe8 Nxd1 34. a4 Nxc3 35. a5 Nb5}]
\mainline{%
29... Rd8 30. Qf5 30... Qa3 31. Rb7?? } [\movecomment{%
31. Rd1 Qxa2 32. Nc5 Qa5 33. Rxd3 Rxd3 34. Qxd3 Qxc5 35. Qd4 Qc6 36. c4 g6 37. Qd5 Qxd5}]
\mainline{%
31... Qxa2 32. Nd6?! } [\movecomment{%
32. Re7 Qb1+ 33. Kg2 Rf8 34. Nd6 Ne1+ 35. Kh3 Qxf5+ 36. Nxf5 Nd3 37. Kg2 Ra8 38. Re3 Nc5}]
\mainline{%
32... Qxf2+ 33. Qxf2 33... Nxf2 34. Kxf2 34... Rxd6 35. c4 35... Rd2+ 36. Kg1 36... Rc2 37. Rc7 37... g5 38. c5 38... Kg7 39. c6 39... Kf6 40. Rc8 40... Kf5 41. c7 41... Kg4 42. h4?? } [\movecomment{%
42. Rh8 Rxc7 43. Rxh6 f5 44. Rb6 Rc1+ 45. Kg2 Rc2+ 46. Kg1}]
\mainline{%
42... Kxg3 43. Kf1 43... Kxh4 44. Ke1 44... f5 45. Kd1 45... Rc6 46. Kd2 46... Kg3 47. Kd3 47... f4 48. Kd4 48... f3 49. Kd5 49... Rc2 50. Kd6 50... f2 51. Rf8 51... Kg2 52. c8Q 52... Rxc8 53. Rxc8 53... f1Q 54. Rc1?! } [\movecomment{%
54. Ke7 Qe2+ 55. Kd8 Qd3+ 56. Ke7 Qe3+ 57. Kd6 Qa3+ 58. Kd5 Qf3+ 59. Kd6 Qf6+ 60. Kc7 Qc3+}]
\mainline{%
54... Qxc1 55. Ke6 55... Qf4 56. Kd5 56... Kf3 57. Ke6 57... Ke4 58. Kd7 58... Qe5 59. Kc6 59... Qd4 60. Kb5 60... Qc3 61. Kb6 61... Qc4 62. Kb7 62... Qc5 63. Kb8 63... Qc6 64. Ka7 64... Qb5 65. Ka8 65... Kd5 66. Ka7 66... Kc6 67. Ka8 67... Qb7\mate{}}\rbwins



==> chess_examples/pgn2latexENG.tex <==

\begin{document}%
%\cleardoublepage

\tableofcontents
\cleardoublepage

\begin{multicols*}{2}
\chapter{}
This is a chapter created by pgn2latex.
\include{pgn2latex_out}

\end{multicols*}

\cleardoublepage
\printindex
\printindex[players]
\printindex[positions]

\end{document}

==> chess_examples/pgn2latex_out.tex <==
\newgame
\resetPgnTags
\def\Event{}
\def\Site{}
\def\Date{}
\def\WhitePlayer{Human}
\def\BlackPlayer{Transfer Maia}
\def\Result{\whiteWins}
\gameHeader

\firstmainline[level=1]{1. e4 e6 2. d4 d5 3. Nc3 Nf6 4. Bg5 Be7 5. e5 Nfd7 6. h4 c5?! }
 (0.12 {\withinit} 0.70) Inaccuracy. Bxg5 was best. 

 C13 French Defense: Alekhine-Chatard Attack, Breyer Variation 

\variation[level=2]{6... Bxg5 7. hxg5 Qxg5 8. Nh3 Qh4 9. g3 Qe7 10. Qg4 g6 11. O-O-O}

\mainline[level=1]{ 7. Nb5?? }
 (0.70 {\withinit} -1.72) Blunder. Bxe7 was best. 

\variation[level=2]{7. Bxe7 Kxe7 8. f4 Nc6 9. dxc5 Nxc5 10. a3 a5 11. Qg4 Nd4}

\mainline[level=1]{ 7... O-O?? }
 (-1.72 {\withinit} 1.16) Blunder. f6 was best. 

\variation[level=2]{7... f6 8. exf6 Nxf6 9. dxc5 O-O 10. Nf3 Bxc5 11. Qd2 Qb6 12. b4}

\mainline[level=1]{ 8. Bxe7 Qxe7 9. Nc7 Nc6 10. Nxa8 Nxd4 11. c3 Nc6 12. f4 f6 13. exf6? }
 (0.95 {\withinit} -0.07) Mistake. Nf3 was best. 

\variation[level=2]{13. Nf3 fxe5}

\mainline[level=1]{ 13... Nxf6 14. Nf3 Nh5?? }
 (-0.69 {\withinit} 1.94) Blunder. e5 was best. 

\variation[level=2]{14... e5 15. Be2}

\mainline[level=1]{ 15. Qd2 Nxf4 16. O-O-O Bd7?! }
 (2.29 {\withinit} 3.55) Inaccuracy. c4 was best. 

\variation[level=2]{16... c4 17. Re1}

\mainline[level=1]{ 17. Nc7 Qd6 18. Nb5 Qb8 19. Bd3 a6 20. Na3 b5 21. Ng5 h6 22. Nf3?! }
 (2.87 {\withinit} 1.90) Inaccuracy. Bh7+ was best. 

\variation[level=2]{22. Bh7+}

\mainline[level=1]{ 22... b4 23. cxb4?! }
 (1.70 {\withinit} 1.08) Inaccuracy. Nc2 was best. 

\variation[level=2]{23. Nc2 c4}

\mainline[level=1]{ 23... Nxb4 24. Bb1 e5 25. Rhe1?? }
 (1.52 {\withinit} -2.75) Blunder. g3 was best. 

\variation[level=2]{25. g3}

\mainline[level=1]{ 25... e4 26. Ng1? }
 (-1.95 {\withinit} -3.75) Mistake. Qc3 was best. 

\variation[level=2]{26. Qc3}

\mainline[level=1]{ 26... Qe5?? }
 (-3.75 {\withinit} 2.32) Blunder. Bg4 was best. 

\variation[level=2]{26... Bg4 27. Nh3 Nbd3+ 28. Bxd3 Nxd3+ 29. Kb1 Bxd1 30. Rxd1 c4 31. Qc2 Kh8 32. Ka1 Qe5 33. Nb1}

\mainline[level=1]{ 27. Qc3?? }
 (2.32 {\withinit} -0.87) Blunder. g3 was best. 

\variation[level=2]{27. g3 Ne6 28. Nc4 Qc7 29. Rxe4 dxe4 30. Qxd7 Nd3+ 31. Rxd3 Rf1+ 32. Kd2 exd3 33. Qxe6+ Qf7}

\mainline[level=1]{ 27... Qxc3+?? }
 (-0.87 {\withinit} 1.39) Blunder. Qb8 was best. 

\variation[level=2]{27... Qb8 28. Nc4}

\mainline[level=1]{ 28. bxc3 Nbd3+ 29. Bxd3 Nxd3+ 30. Kd2 Rf2+?! }
 (0.82 {\withinit} 1.86) Inaccuracy. Bg4 was best. 

\variation[level=2]{30... Bg4 31. Ke3}

\mainline[level=1]{ 31. Re2 Bg4?? }
 (2.34 {\withinit} 5.38) Blunder. Rf4 was best. 

\variation[level=2]{31... Rf4 32. Nh3}

\mainline[level=1]{ 32. Rxf2 Nxf2 33. Rb1 d4 34. Rb8+ Kh7 35. cxd4 cxd4 36. Nc4 e3+?! }
 (4.55 {\withinit} 6.26) Inaccuracy. Be6 was best. 

\variation[level=2]{36... Be6 37. Ne5 Bxa2 38. Rd8 e3+ 39. Ke2 Ne4 40. Rxd4 Ng3+ 41. Ke1 Nf5 42. Rf4 Nd6 43. Ra4}

\mainline[level=1]{ 37. Nxe3 dxe3+ 38. Kxe3 Nd1+ 39. Kd2 Nf2 40. Re8 Kg6 41. Nf3 Kf7 42. Re2 Nh1 43. Ne5+ Kf6 44. Nxg4+ Kf5 45. Ne3+ Kf4 46. Nd5+ Kg3 47. Re7 Kxh4?? }
 (6.71 {\withinit} Mate in 9) Checkmate is now unavoidable. Kxg2 was best. 

\variation[level=2]{47... Kxg2 48. Rxg7+}

\mainline[level=1]{ 48. Rxg7 Ng3 49. Rg6 h5?! }
 (60.47 {\withinit} Mate in 15) Checkmate is now unavoidable. Nf5 was best. 

\variation[level=2]{49... Nf5 50. Ne3}

\mainline[level=1]{ 50. Rxa6? }
 (Mate in 15 {\withinit} 9.32) Lost forced checkmate sequence. Ne3 was best. 

\variation[level=2]{50. Ne3 Ne4+ 51. Kd3 Ng5 52. a4 Kg3 53. Rxg5+ Kf4 54. Rf5+ Kg3 55. Rf6 a5 56. Rf5 Kh4}

\mainline[level=1]{ 50... Kg4 51. Ne3+ Kf4 52. Ra4+ Ke5 53. Ra5+ Kf4 54. a4 Ne4+ 55. Ke2 Nc3+ 56. Kd3 Ne4?! }
 (60.67 {\withinit} Mate in 9) Checkmate is now unavoidable. Na2 was best. 

\variation[level=2]{56... Na2 57. Rf5+}

\mainline[level=1]{ 57. Rxh5?! }
 (Mate in 9 {\withinit} 76.34) Lost forced checkmate sequence. Rf5+ was best. 

\variation[level=2]{57. Rf5+ Kg3 58. Kxe4 Kh4 59. a5 Kg3 60. a6 Kh4 61. a7 Kg3 62. a8=Q Kh4 63. Qa1 Kg3}

\mainline[level=1]{ 57... Ng3?! }
 (76.34 {\withinit} Mate in 12) Checkmate is now unavoidable. Nd6 was best. 

\variation[level=2]{57... Nd6 58. a5 Kg3 59. Nf5+ Kg4 60. Nxd6 Kxh5 61. a6 Kg5 62. a7 Kf6 63. a8=Q Ke6 64. Ne4}

\begin{samepage}\mainline[level=1]{ 58. Rh4+ Ke5 59. a5 Nf5 60. Rh5 Ke6 61. Rxf5 Kd6 62. a6 Kc7 63. a7 Kb7 64. Rf7+ Ka8 65. Rf6 Kxa7 66. Kc4 Kb7 67. Kd5 Kc7 68. g4 Kd7 69. g5 Ke7 70. Ke5 Kd7 71. Nd5 Ke8 72. Kd6 Kd8 73. Rf8# }
 White wins by checkmate. 
 \rwwins\end{samepage}

\newgame
\resetPgnTags
\def\Event{}
\def\Site{}
\def\Date{}
\def\WhitePlayer{Transfer Maia}
\def\BlackPlayer{Human}
\gameHeader

\firstmainline[level=1]{1. e4 a6 }
 B00 St. George Defense 

\mainline[level=1]{ 2. d4 b5 3. Nf3 Bb7 4. Nc3? }
 (0.68 {\withinit} -0.39) Mistake. Bd3 was best. 

\variation[level=2]{4. Bd3 e6 5. O-O c5 6. c3 cxd4 7. cxd4 Nf6 8. Nbd2 Be7}

\mainline[level=1]{ 4... b4 5. Nd5 e6 6. Nf4 Bxe4 7. Bd3 Nf6 8. O-O Be7 9. Re1 Bxd3 10. Qxd3 O-O 11. Bd2 Nc6?! }
 (-1.63 {\withinit} -0.96) Inaccuracy. a5 was best. 

\variation[level=2]{11... a5 12. a3 bxa3 13. bxa3 h6 14. Rab1 d6 15. Qb5 Qd7 16. c4 Qxb5 17. Rxb5 a4 18. Reb1}

\mainline[level=1]{ 12. Rad1?! }
 (-0.96 {\withinit} -1.61) Inaccuracy. d5 was best. 

\variation[level=2]{12. d5}

\mainline[level=1]{ 12... a5? }
 (-1.61 {\withinit} -0.43) Mistake. Bd6 was best. 

\variation[level=2]{12... Bd6 13. c4 bxc3 14. bxc3 Rb8 15. Bc1 a5 16. c4 Bb4 17. Rf1 d5 18. Ne5 dxc4 19. Qxc4}

\mainline[level=1]{ 13. c4? }
 (-0.43 {\withinit} -1.81) Mistake. d5 was best. 

\variation[level=2]{13. d5 Nb8}

\mainline[level=1]{ 13... bxc3 14. Bxc3? }
 (-1.43 {\withinit} -2.84) Mistake. bxc3 was best. 

\variation[level=2]{14. bxc3 d5 15. Ng5 Bd6 16. Nh5 g6 17. Nf4 Re8 18. Qh3 Rb8 19. Nd3 e5 20. Nxe5 Nxe5}

\mainline[level=1]{ 14... Re8?! }
 (-2.84 {\withinit} -2.12) Inaccuracy. Nb4 was best. 

\variation[level=2]{14... Nb4}

\mainline[level=1]{ 15. d5 exd5?? }
 (-1.97 {\withinit} 0.07) Blunder. Nb4 was best. 

\variation[level=2]{15... Nb4 16. Bxb4 axb4 17. dxe6 fxe6 18. Qc4 Bd6 19. Nd3 Nd5 20. Nde5 c6 21. Re2 Rf8 22. g3}

\mainline[level=1]{ 16. Nxd5 Nxd5 17. Qxd5 Bd6?? }
 (0.04 {\withinit} 4.77) Blunder. h6 was best. 

\variation[level=2]{17... h6 18. Ne5 Nxe5 19. Qxe5 Bf6 20. Qxe8+ Qxe8 21. Rxe8+ Rxe8 22. Bxa5 Bxb2 23. Rxd7 Ra8 24. Bxc7}

\mainline[level=1]{ 18. Rxe8+?? }
 (4.77 {\withinit} 0.52) Blunder. Ng5 was best. 

\variation[level=2]{18. Ng5 Rf8}

\mainline[level=1]{ 18... Qxe8 19. Re1 Qf8?! }
 (0.37 {\withinit} 0.95) Inaccuracy. Ne7 was best. 

\variation[level=2]{19... Ne7}

\mainline[level=1]{ 20. Ng5? }
 (0.95 {\withinit} -0.32) Mistake. Qf5 was best. 

\variation[level=2]{20. Qf5 Ne7 21. Qxd7 a4 22. a3 Nd5 23. Ba5 Nb6 24. Qc6 Bc5 25. Bxb6 cxb6 26. Re4 Qd8}

\mainline[level=1]{ 20... h6 21. Ne4 Re8 22. g3?! }
 (0.00 {\withinit} -0.77) Inaccuracy. Kf1 was best. 

\variation[level=2]{22. Kf1 Re6 23. a3 Qb8 24. Nxd6 Rxd6 25. Qc4 Re6 26. Rxe6 fxe6 27. Qd3 Qe8 28. Qa6 Qb8}

\mainline[level=1]{ 22... Nb4?? }
 (-0.77 {\withinit} 1.00) Blunder. Re7 was best. 

\variation[level=2]{22... Re7 23. Kf1}

\mainline[level=1]{ 23. Qd4?! }
 (1.00 {\withinit} 0.00) Inaccuracy. Qxa5 was best. 

\variation[level=2]{23. Qxa5}

\mainline[level=1]{ 23... Be5 24. Qxd7 Bxc3??\dia}
{\par \centering\chessboardn \par}
 (0.10 {\withinit} 5.25) Blunder. Re7 was best. 

\variation[level=2]{24... Re7 25. Qd2 Bxc3 26. Nxc3 Rxe1+ 27. Qxe1 Qd8 28. Qe4 c6 29. a3 Nd3 30. Qxc6 Nxb2 31. Qe4}

\mainline[level=1]{ 25. bxc3?? }
 (5.25 {\withinit} 1.04) Blunder. Nf6+ was best. 

\variation[level=2]{25. Nf6+}

\mainline[level=1]{ 25... Rd8 26. Qxc7 Nd3 27. Rb1?? }
 (1.78 {\withinit} -0.04) Blunder. Rd1 was best. 

\variation[level=2]{27. Rd1}

\mainline[level=1]{ 27... Rc8?? }
 (-0.04 {\withinit} 2.12) Blunder. f5 was best. 

\variation[level=2]{27... f5 28. Nd2 Nxf2 29. Nf3 Nh3+ 30. Kg2 Ng5 31. Nd4 Rc8 32. Qd7 Rxc3 33. Rb7 Qf6 34. Qxf5}

\mainline[level=1]{ 28. Qxa5 Ra8? }
 (2.46 {\withinit} 4.63) Mistake. Qe7 was best. 

\variation[level=2]{28... Qe7 29. Qf5}

\mainline[level=1]{ 29. Qd5?! }
 (4.63 {\withinit} 3.09) Inaccuracy. Qb5 was best. 

\variation[level=2]{29. Qb5 Rd8 30. Rd1 Qe8 31. Qxe8+ Rxe8 32. Nd6 Nb2 33. Nxe8 Nxd1 34. a4 Nxc3 35. a5 Nb5}

\mainline[level=1]{ 29... Rd8 30. Qf5 Qa3 31. Rb7?? }
 (3.22 {\withinit} 0.54) Blunder. Rd1 was best. 

\variation[level=2]{31. Rd1 Qxa2 32. Nc5 Qa5 33. Rxd3 Rxd3 34. Qxd3 Qxc5 35. Qd4 Qc6 36. c4 g6 37. Qd5 Qxd5}

\mainline[level=1]{ 31... Qxa2 32. Nd6?! }
 (0.88 {\withinit} 0.19) Inaccuracy. Re7 was best. 

\variation[level=2]{32. Re7 Qb1+ 33. Kg2 Rf8 34. Nd6 Ne1+ 35. Kh3 Qxf5+ 36. Nxf5 Nd3 37. Kg2 Ra8 38. Re3 Nc5}

\mainline[level=1]{ 32... Qxf2+ 33. Qxf2 Nxf2 34. Kxf2 Rxd6 35. c4 Rd2+ 36. Kg1 Rc2 37. Rc7 g5 38. c5 Kg7 39. c6 Kf6 40. Rc8 Kf5 41. c7 Kg4 42. h4?? }
 (0.00 {\withinit} -8.36) Blunder. Rh8 was best. 

\variation[level=2]{42. Rh8 Rxc7 43. Rxh6 f5 44. Rb6 Rc1+ 45. Kg2 Rc2+ 46. Kg1}

\mainline[level=1]{ 42... Kxg3 43. Kf1 Kxh4 44. Ke1 f5 45. Kd1 Rc6 46. Kd2 Kg3 47. Kd3 f4 48. Kd4 f3 49. Kd5 Rc2 50. Kd6 f2 51. Rf8 Kg2 52. c8=Q Rxc8 53. Rxc8 f1=Q 54. Rc1?! }
 (-59.95 {\withinit} Mate in 9) Checkmate is now unavoidable. Ke7 was best. 

\variation[level=2]{54. Ke7 Qe2+ 55. Kd8 Qd3+ 56. Ke7 Qe3+ 57. Kd6 Qa3+ 58. Kd5 Qf3+ 59. Kd6 Qf6+ 60. Kc7 Qc3+}

\begin{samepage}\mainline[level=1]{ 54... Qxc1 55. Ke6 Qf4 56. Kd5 Kf3 57. Ke6 Ke4 58. Kd7 Qe5 59. Kc6 Qd4 60. Kb5 Qc3 61. Kb6 Qc4 62. Kb7 Qc5 63. Kb8 Qc6 64. Ka7 Qb5 65. Ka8 Kd5 66. Ka7 Kc6 67. Ka8 Qb7# }
 Black wins by checkmate. 
 \rbwins\end{samepage}



==> tables/perplexity.tex <==
\begin{table}[t]
\centering
    \begin{tabular}{lrr}
    \toprule
    {} &  perplex\_trans &  perplex\_maia \\
    player\_count &                &               \\
    \midrule
    20000        &       1.967156 &      2.151236 \\
    30000        &       1.934596 &      2.143282 \\
    40000        &       1.884081 &      2.110341 \\
    \bottomrule
    \end{tabular}
    \caption{Perplexity for the different player counts}
\end{table}

==> tables/train_test_split.tex <==
\begin{tabular}{rll}
\toprule
 Min games &  explore/holdout &  validatation \\
\midrule
     10000 &              233 &          1866 \\
     20000 &               36 &           295 \\
     30000 &               10 &            86 \\
     40000 &               10 &            19 \\
\bottomrule
\end{tabular}

